Language Models can Solve Computer Tasks

Agents capable of carrying out general tasks on a computer can improve efficiency and productivity by automating repetitive tasks and assisting in complex problem-solving. Ideally, such agents should be able to solve new computer tasks presented to them through natural language commands. However, previous approaches to this problem require large amounts of expert demonstrations and task-specific reward functions, both of which are impractical for new tasks. In this work, we show that a pre-trained large language model (LLM) agent can execute computer tasks guided by natural language using a simple prompting scheme where the agent Recursively Criticizes and Improves its output (RCI). The RCI approach significantly outperforms existing LLM methods for automating computer tasks and surpasses supervised learning (SL) and reinforcement learning (RL) approaches on the MiniWoB++ benchmark. We compare multiple LLMs and find that RCI with the InstructGPT-3+RLHF LLM is state-of-the-art on MiniWoB++, using only a handful of demonstrations per task rather than tens of thousands, and without a task-specific reward function. Furthermore, we demonstrate RCI prompting's effectiveness in enhancing LLMs' reasoning abilities on a suite of natural language reasoning tasks, outperforming chain of thought (CoT) prompting with external feedback. We find that RCI combined with CoT performs better than either separately. Our code can be found here: https://github.com/posgnu/rci-agent.

==> tables/ablating_rci.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]
\centering
\scriptsize
\begin{tabular}{lrrrrr}\toprule
& &click-checkboxes-large &click-menu &enter-text \\\midrule
\multirow{2}{*}{Explicit RCI} &0 &0.9 &0.9 &0.9 \\
&1 &0.9 &0.9 &0.9 \\\midrule
\multirow{3}{*}{Implicit RCI} &0 &0.9 &0.9 &0.9 \\
&1 &0.9 &0.9 &0.9 \\
&2 &0.9 &0.9 &0.9 \\
\bottomrule
\end{tabular}
\caption{The number of loops in self-play prompting affects the grounding improvement and increases the success rate in tasks with three different difficulties. (placeholder)}\label{tab:rci_ablate}
\end{table}

==> tables/prompt_table.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{p{\textwidth}}\hline

    \hline
    \end{tabular}
    \caption{The base prompts used for all tasks.}
    \label{tab:my_label}
\end{table}
